StructRe: Rewriting for Structured Shape Modeling

Man-made 3D shapes are naturally organized in parts and hierarchies; such structures provide important constraints for shape reconstruction and generation. Modeling shape structures is difficult, because there can be multiple hierarchies for a given shape, causing ambiguity, and across different categories the shape structures are correlated with semantics, limiting generalization. We present StructRe, a structure rewriting system, as a novel approach to structured shape modeling. Given a 3D object represented by points and components, StructRe can rewrite it upward into more concise structures, or downward into more detailed structures; by iterating the rewriting process, hierarchies are obtained. Such a localized rewriting process enables probabilistic modeling of ambiguous structures and robust generalization across object categories. We train StructRe on PartNet data and show its generalization to cross-category and multiple object hierarchies, and test its extension to ShapeNet. We also demonstrate the benefits of probabilistic and generalizable structure modeling for shape reconstruction, generation and editing tasks.

==> fig/5_exp/ablation_iter.tex <==
\begin{figure}
    \centering
    \begin{overpic}  
    [width=\linewidth]{fig/5_exp/ablation_iter_fig.pdf}
       
        \put(5,-1.5){\small input}
        \put(24,-1.5){\small GT parts}
        \put(46,-1.5){\small step 0}
        \put(66,-1.5){\small step 1}
        \put(86,-1.5){\small step 2}
    \end{overpic}

    \caption{\textbf{Example of iterative decoding}. Given the point cloud input, our model can first detect parts and then gradually remove redundant and extraneous parts via iterative decoding (See the marked regions by arrows).}
    \label{fig:ablation_iter}
\end{figure}

==> fig/5_exp/ablation_unistruct.tex <==
\begin{figure}
    \centering
    \begin{overpic}[width=0.85\linewidth]{fig/5_exp/ablation_unistruct_fig_v4.pdf}
        \put(5,1){input}
        \put(24,1){w/o inp}
        \put(43,1){w/ inp: 0\%}
        \put(63,1){w/ inp: 25\%}
        \put(82,1){w/ inp: 50\%}
        
    \end{overpic}
    
    \caption{\textbf{Visualization of ablation on input conditioning for part shape reconstruction}. }
    \label{fig:ablation_unistruct}
\end{figure}

==> morefig/fig/ablation_mapping_v1.tex <==
\begin{figure*}
    \centering
    \begin{overpic}
        [width=\linewidth]{morefig/fig/ablation_mapping_fig2.pdf}
        \put(7,0){\small input}
        \put(23,0){\small GT part}
        \put(41,0){\small full}
        \put(55,0){\small w/o aug}
        \put(71.5,0){\small w/o iter}
        \put(88,0){\small w/o inp}
		\put(0,56){\small \bfseries(a)}
		\put(0,40){\small \bfseries(b)}
		\put(0,24){\small \bfseries(d)}
		\put(0,11){\small \bfseries(d)}
    \end{overpic}
    \caption{
    \textbf{Examples of ablation results}. Compared to our full model, the variations on data augmentation, iterative decoding and input geometry conditioning can produce less accurate results with missing, duplicated or distorted parts.
    }
    \label{fig:ablation_mapping_v1}
\end{figure*}

==> morefig/fig/diffnoise_gen.tex <==
\begin{figure*}
    \centering
    % \includegraphics
    \begin{overpic}
        [width=\linewidth]{morefig/fig/diffnoise_gen_fig2.pdf}
        \put(-1,-2){(a) condition}
        \put(12,-2){(b) 0.4}
        \put(22,-2){(c) 0.8}
        \put(32,-2){(d) 1.2}
        \put(42,-2){(e) 1.6}

        \put(51,-2){(a) condition}
        \put(63,-2){(b) 0.4}
        \put(73,-2){(c) 0.8}
        \put(83,-2){(d) 1.2}
        \put(93,-2){(e) 1.6}
    \end{overpic}
    % \vspace{1pt}
     \vspace{0.1pt}
    \caption{
    \textbf{Shape-conditioned generation with different noise levels}. Given conditioned shapes (a), our model can generate diverse structured shapes with different noise levels (b-f). The numbers indicate the noise levels.
    }
    \label{fig:diffnoise_gen}
\end{figure*}














==> morefig/fig/method_step_vis.tex <==
% A "teaser" figure, centered below the title and authors and above the body of the work.
\begin{figure*}[h]
  \centering
  \begin{overpic}[width=0.95\linewidth]{morefig/fig/method_step_group.pdf}
          \put(2.5, 36){\textcolor{red}{$d_0$}}
          \put(35.5, 36){\textcolor{red}{$d_0$}}
          \put(68.5, 36){\textcolor{red}{$d_0$}}
    
          \put(3, 7){\textcolor{red}{$d_1$}}
          \put(35.5, 7){\textcolor{red}{$d_1$}}
          \put(68.5, 7){\textcolor{red}{$d_1$}}
          
        \put(14, 28){(a) level 0}
        \put(47, 28){(b) level 1}
        \put(80, 28){(c) level 2}

        \put(14, -2){(f) level 0}
        \put(47, -2){(e) level 1}
        \put(80, -2){(d) level 2}       
  \end{overpic}

    \caption{
    \textbf{Detailed rewriting process.} Starting from a point cloud input, (a) \(\rightarrow\) (c) illustrate the structured reconstruction process (level 0 \(\rightarrow\) level 2). Conditioned on a shape, (d) \(\rightarrow\) (f) show the generation process (level 2 \(\rightarrow\) level 0). In each sub-figure, the bottom-left corner shows the model input, while the top-right corner shows the output.  }
  \label{fig:method_step_vis}
\end{figure*}


==> morefig/fig/more_editting.tex <==
\begin{figure*}
    \centering
    \begin{overpic}
        [width=\linewidth]{morefig/fig/more_editing_fig2.pdf}
          \put(-1, 41){\rotatebox{90}{\small \textbf{(a) microwave}}}
          \put(-1, 30){\rotatebox{90}{\small \textbf{(b) mug}}}
          \put(-1, 17){\rotatebox{90}{\small \textbf{(c) chair}}}
          \put(-1, 1){\rotatebox{90}{\small \textbf{(d) display}}}

          \put(3,29){(1) input}
          \put(17,29){(2) level 0}
          \put(29,29){(3) part swapping}
          \put(46,29){(4) level 1}
          \put(57,29){(5) zoom-in}
          \put(74,29){(6) failure case}

          
          \put(3,-1){(1) input}
          \put(17,-1){(2) level 0}
          \put(32,-1){(3) level 1}
          \put(46,-1){(4) level 2}
          \put(60,-1){(5) level 3}
          \put(72,-1){(6) part swapping}
          \put(90,-1){(7) level 4}
    \end{overpic}
    \caption{
    \textbf{More examples of shape editing}.
    (a) Microwave edited to integrate a mug handle;
    (b) Mug with the removal of its handle;
    (c) Chair with its star-shaped leg base replaced by a display screen support base;
    (d) Display modified by replacing its support base with a chair’s star-shaped leg base with wheels.
    Note that (a)(6)$\rightarrow$(b)(6) shows a failure case of part editing due to unreasonable part initialization.
    }
    \label{fig:more_editting}
\end{figure*}

==> morefig/fig/segmentation.tex <==
\begin{figure*}[h]
    \centering
    \begin{overpic}
        [width=0.8\linewidth]{morefig/fig/segmentation_fig.pdf}

        \put(5,0){input}
        \put(16,0){prediction}
        \put(30,0){segmentation}

        \put(52,0){input}
        \put(67,0){prediction}
        \put(83,0){segmentation}

    \end{overpic}
    \caption{
        \textbf{Point cloud segmentation} by projecting points onto the predicted parts. 
    }
    \label{fig:segmentation}
\end{figure*}

==> morefig/fig/uncond_gen_all.tex <==
\begin{figure*}
    \centering
    \begin{overpic}
        [width=\linewidth]{morefig/fig/uncond_gen_all_fig.pdf}
        \put(15,87){bowl}
        \put(42,87){bottle}
        \put(70, 87){bag}
        
        \put(20,76){bed}
        \put(50,76){trash-can}
        \put(68,76){faucet}

        \put(20, 65){scissors}
        \put(48,63){refrigerator}
        \put(70,65){clock}


        \put(23,51){laptop}
        \put(62,51){display}

        \put(12, 38){mug}
        \put(30,38){hat}
        \put(57,38){knife}

        \put(30,26.5){vase}
        \put(63,26.5){hat}
        
        \put(3, 13){dishwasher}
        \put(22,13){earphone}
        \put(57,13){door}
        
        \put(17, 2){keyboard}
        \put(57,2){microwave}
       
    \end{overpic}

    \caption{
    \textbf{Gallery of category-conditioned generation on small categories.} We present generation results for the remaining categories in PartNet, excluding Chair, Cabinet, and Table.
    }
    \label{fig:uncond_gen_all}
\end{figure*}

==> morefig/table/shape_uncond_gen_train.tex <==
\begin{table}[h]
\fontsize{8}{12}\selectfont
  \centering
  \caption{ 
  \textbf{Comparison of structured shape generation against training set}. StructureNet trains specific models for each object category, while our model is evaluated across categories. Note that our results are generated using the category-conditioned setting (Sec.~6.4.1 in the main text).
  }
    \begin{tabular}{ccrrr}
    \toprule[1pt]
    \textbf{Category} & \textbf{Method} & \textbf{FPD}$\downarrow$ & \textbf{COV}$\downarrow$ & \textbf{MMD} $\downarrow$\\
    
    \midrule
    \multirow{2}[2]{*}{Chair}  & StructureNet	  &  4.11	  &0.92& \textbf{0.54} \\
& Ours & \textbf{2.62} &  \textbf{0.87} & 0.80 \\

    \midrule
    \multirow{2}[2]{*}{Table} & StructureNet	  & 5.48 & 1.46 &  \textbf{0.50} \\
& Ours	   & \textbf{2.36} & \textbf{0.83} & 0.71 \\

    \midrule
    \multirow{2}[2]{*}{Cabinet} & StructureNet	  & 6.79 & 1.13 & \textbf{0.59} \\
& Ours	   &  \textbf{2.92} & \textbf{0.57} & 0.71  \\



    \bottomrule[1pt]
    \end{tabular}
  \label{tab:eval_shape_gen_train_set}%
  \vspace{0mm}
\end{table}

==> table/ablation_chair.tex <==
\begin{table}[t]
\fontsize{8}{12}\selectfont
  \centering
  \caption{
  \textbf{Ablation study}. Data obtained on the whole chair test set. CD is squared chamfer distance in the scale of $\times 10^{-3}$. EMD is squared Earth's mover distance in the scale of $\times 10^{-2}$. 
  }
    \begin{tabular}{cccccccc}
    \toprule[1pt]       
    \textbf{Config} & \textbf{Iter} & \textbf{Aug}  & \textbf{Inp}  &  & \textbf{CD} $\downarrow$ & \textbf{EMD} $\downarrow$ & \textbf{Hier} $\downarrow$\\
    \midrule
    w/o aug  & \checkmark &     &   \checkmark &        & 3.5  &  0.65  &  0.348 \\
    w/o iter &  &  \checkmark  &   \checkmark&          & 1.3  &  0.42  &  0.463 \\
    w/o inp  & \checkmark &  \checkmark  &    &         & 1.4  &  0.40  &  0.219 \\
    full     & \checkmark & \checkmark & \checkmark&    & \textbf{1.2}  &  \textbf{0.38}  &  \textbf{0.207} \\
    \bottomrule[1pt]
    \end{tabular}
  \label{tab:ablation_chair}
  % \vspace{-4mm}
\end{table}

==> table/ablation_unistruct.tex <==
\begin{table}[t]
\fontsize{8}{12}\selectfont
  \centering
  \caption{\textbf{Ablation of input conditioning on part shape reconstruction}, evaluated on chair test data. }
    \begin{tabular}{ccccccc}
    \toprule[1pt]
    \multirow{2}[4]{*}{\textbf{Metric}} & \multirow{2}[4]{*}{\textbf{w/o inp}} & \multicolumn{5}{c}{\textbf{w/ inp}} \\
    \cmidrule{3-7}          &       & 0\% & 25\% & 50\% &  75\% & 100\%\\
    
    \midrule

    \textbf{CD}{\scriptsize$\times 10^{-2}$}$\downarrow$ & 0.23 & 0.24 & 0.20 & 0.20 & 0.20 & 0.20 \\
    \textbf{F1}$\uparrow$ & 0.98 & 0.98 & 0.99 & 0.99 & 0.99 & 0.99  \\

    \bottomrule[1pt]
    \end{tabular}%
  \label{tab:ablation_unistruct}%
  \vspace{-2mm}
\end{table}%
